Measurements of the Absolute Branching Ratios for the Dominant KL Decays, the KL Lifetime, and Vus with the KLOE Detector

From a sample of about 10^9 Phi mesons produced at DAFNE, we have selected KL mesons tagged by observing KS->pi+pi- decays. We present results on the major KL branching ratios, including those of the semileptonic decays needed for the determination of Vus. These branching ratio measurements are fully inclusive with respect to final-state radiation. The KL lifetime has also been measured.

==> macro.tex <==

% Macros: Sectioning

\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[1]{Eqs.~(\ref{#1})}
\newcommand{\andEq}[1]{and~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Ref}[1]{Ref.~\citen{#1}}
\newcommand{\Refs}[1]{Refs.~\citen{#1}}
\newcommand{\andRef}[1]{and~\citen{#1}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Secs}[1]{Secs.~\ref{#1}}
\newcommand{\andSec}[1]{and~\ref{#1}}
\newcommand{\Tab}[1]{Tab.~\ref{#1}}


% Macros: Abbreviations

\newcommand{\apriori}{{\em a priori}}
\newcommand{\DAFNE}{DA$\Phi$NE}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\eg}{{\em e.g.}}
\newcommand{\etseq}{{\em et seq.}}
\newcommand{\ith}{\ensuremath{i^\mathrm{th}}}
\newcommand{\perse}{{\em per se}}


% Macros: Units

\newcommand{\cm}{\ensuremath{\mathrm{cm}}}
\newcommand{\Deg}{\ensuremath{^\circ}}
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}}
\newcommand{\GeVcc}{\ensuremath{\mathrm{GeV}}}
\newcommand{\KG}{\ensuremath{\mathrm{kG}}}
\newcommand{\Lpb}{\ensuremath{\mathrm{pb}^{-1}}}
\newcommand{\Lfb}{\ensuremath{\mathrm{fb}^{-1}}}
\newcommand{\Lcms}{\ensuremath{\mathrm{cm}^{-2}\,\mathrm{s}^{-1}}}
\newcommand{\MeV}{\ensuremath{\mathrm{MeV}}}
\newcommand{\MeVc}{\ensuremath{\mathrm{MeV}}}
\newcommand{\MeVcc}{\ensuremath{\mathrm{MeV}}}
\newcommand{\m}{\ensuremath{\mathrm{m}}}
\newcommand{\mm}{\ensuremath{\mathrm{mm}}}
\newcommand{\mrad}{\ensuremath{\mathrm{mrad}}}
\newcommand{\ns}{\ensuremath{\mathrm{ns}}}
\newcommand{\ps}{\ensuremath{\mathrm{ps}}}
\newcommand{\Tesla}{\ensuremath{\mathrm{T}}}
\newcommand{\um}{\ensuremath{\mu\mathrm{m}}}
\newcommand{\ub}{\ensuremath{\mu\mathrm{b}}}


% Macros: Comparators and operators

\newcommand{\about}{\ensuremath{\sim}}
\newcommand{\geqsim}{\, \raisebox{-0.6ex}{\ensuremath{\stackrel{\textstyle{>}}{\sim}}}\, }
\newcommand{\leqsim}{\, \raisebox{-0.6ex}{\ensuremath{\stackrel{\textstyle{<}}{\sim}}}\, }


% Macros: Functions and symbols with arguments

\newcommand{\BR}[1]{\ensuremath{\mathrm{BR}(#1)}}
\newcommand{\magn}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\mean}[1]{\ensuremath{\left<#1\right>}}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\,\left(#1\right)}}
\newcommand{\Prob}[1]{\ensuremath{\mathrm{Prob}\left(#1\right)}}
\newcommand{\Real}[1]{\ensuremath{\mathrm{Re}\,\left(#1\right)}}
\newcommand{\SN}[2]{\ensuremath{#1\cdot10^{#2}}}
\newcommand{\VS}[2]{\ensuremath{#1\pm#2}}
\newcommand{\VSS}[3]{\ensuremath{#1\pm#2\pm#3}}
\newcommand{\VA}[3]{\ifthenelse{\equal{#2}{#3}}
{\ensuremath{#1\pm#2}}{\ensuremath{#1\,^{+#2}_{-#3}}}}
\newcommand{\Width}[1]{\ensuremath{\Gamma(#1)}}


% Macros: Programs, subprograms, and data structures, with arguments

\newcommand{\Fpack}[1]{\textsc{#1}}
\newcommand{\Fmod}[1]{\textsc{#1}}
\newcommand{\Ffile}[1]{\texttt{#1}}
\newcommand{\Fprog}[1]{\textsc{#1}}
\newcommand{\Ffunc}[1]{\texttt{#1}}
\newcommand{\Fbank}[1]{\texttt{#1}}
\newcommand{\Fdata}[1]{\texttt{#1}}


% Macros: Variables and mathematical expressions

\newcommand{\amu}{\ensuremath{a_\mu}}
\newcommand{\amuHadr}{\ensuremath{a_\mu^\mathrm{had}}}
\newcommand{\CP}{\ensuremath{CP}}
\newcommand{\CPT}{\ensuremath{CPT}}
\newcommand{\eff}{\ensuremath{\varepsilon}}
\newcommand{\Emiss}{\ensuremath{E_\mathrm{miss}}}
\newcommand{\Erad}{\ensuremath{E_\mathrm{rad}}}
\newcommand{\Pmiss}{\ensuremath{P_\mathrm{miss}}}
\newcommand{\Reeps}{\ensuremath{\mathrm{Re}\,(\epsilon'/\epsilon)}}
\newcommand{\Rexp}{\ensuremath{\mathrm{Re}\ x_+}}
\newcommand{\phiP}{\ensuremath{\varphi_P}}
\newcommand{\pstar}{\ensuremath{p^*}}
\newcommand{\pvec}{\ensuremath{\mathbf{p}}}
\newcommand{\rxy}{\ensuremath{r_{xy}}}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}}
\newcommand{\Stat}{\ensuremath{_\mathrm{stat}}}
\newcommand{\Syst}{\ensuremath{_\mathrm{syst}}}
\newcommand{\spi}{\ensuremath{s_\pi}}
\newcommand{\thetaP}{\ensuremath{\theta_P}}
\newcommand{\Vud}{\ensuremath{|V_{ud}|}}
\newcommand{\Vus}{\ensuremath{|V_{us}|}}
\newcommand{\Vusfp}{\ensuremath{|V_{us}|f_+(0)}}
\newcommand{\xvec}{\ensuremath{\mathbf{x}}}


% Macros: Particles and decays

\newcommand{\q}{\ensuremath{q}}
\newcommand{\qbar}{\ensuremath{\bar{q}}}
\newcommand{\qs}{\ensuremath{s}}
\newcommand{\qsbar}{\ensuremath{\bar{s}}}
\newcommand{\qg}{\ensuremath{g}}

\newcommand{\Pazero}{\ensuremath{a_0}}
\newcommand{\Pe}{\ensuremath{e}}
\newcommand{\Pem}{\ensuremath{e^-}}
\newcommand{\Pemp}{\ensuremath{e^\mp}}
\newcommand{\Pep}{\ensuremath{e^+}}
\newcommand{\Peta}{\ensuremath{\eta}}
\newcommand{\Petapr}{\ensuremath{\eta'}}
\newcommand{\Pfzero}{\ensuremath{f_0}}
\newcommand{\Pg}{\ensuremath{\gamma}}
\newcommand{\PK}{\ensuremath{K}}
\newcommand{\PKbar}{\ensuremath{\bar{K}}}
\newcommand{\PKn}{\ensuremath{K^0}}
\newcommand{\PKnbar}{\ensuremath{\bar{K}^0}}
\newcommand{\PKm}{\ensuremath{K^-}}
\newcommand{\PKp}{\ensuremath{K^+}}
\newcommand{\PKpm}{\ensuremath{K^\pm}}
\newcommand{\PKS}{\ensuremath{K_S}}
\newcommand{\PKL}{\ensuremath{K_L}}
\newcommand{\Pmu}{\ensuremath{\mu}}
\newcommand{\Pmump}{\ensuremath{\mu^\mp}}
\newcommand{\Pnu}{\ensuremath{\nu}}
\newcommand{\Pnubar}{\ensuremath{\bar{\nu}}}
\newcommand{\Pomega}{\ensuremath{\omega}}
\newcommand{\Pphi}{\ensuremath{\phi}}
\newcommand{\Ppi}{\ensuremath{\pi}}
\newcommand{\Ppim}{\ensuremath{\pi^-}}
\newcommand{\Ppin}{\ensuremath{\pi^0}}
\newcommand{\Ppip}{\ensuremath{\pi^+}}
\newcommand{\Ppipm}{\ensuremath{\pi^\pm}}
\newcommand{\Prho}{\ensuremath{\rho}}
\newcommand{\Prhop}{\ensuremath{\rho^+}}
\newcommand{\Prhom}{\ensuremath{\rho^-}}
\newcommand{\Prhon}{\ensuremath{\rho^0}}
\newcommand{\Ptau}{\ensuremath{\tau}}

\newcommand{\Dazeroetapin}{\ensuremath{a_0\rightarrow\eta\pi^0}}

\newcommand{\Detagg}{\ensuremath{\eta\rightarrow\gamma\gamma}}
\newcommand{\Detapippimpin}{\ensuremath{\eta\rightarrow\pi^+\pi^-\pi^0}}
\newcommand{\Detapretapippim}{\ensuremath{\eta'\rightarrow\eta\pi^+\pi^-}}

\newcommand{\Dfzeropippim}{\ensuremath{f_0\rightarrow\pi^+\pi^-}}
\newcommand{\Dfzeropinpin}{\ensuremath{f_0\rightarrow\pi^0\pi^0}}

\newcommand{\DKeIII}{\ensuremath{K_{e3}}}
\newcommand{\DKlIII}{\ensuremath{K_{\ell3}}}
\newcommand{\DKeIIIp}{\ensuremath{K^+_{e3}}}
\newcommand{\DKeIIIn}{\ensuremath{K^0_{e3}}}
\newcommand{\DKmuIII}{\ensuremath{K_{\mu 3}}}
\newcommand{\DKpipi}{\ensuremath{K\rightarrow\pi\pi}}
\newcommand{\DKpipipi}{\ensuremath{K\rightarrow3\pi}}

\newcommand{\DKLgg}{\ensuremath{K_L\rightarrow\gamma\gamma}}
\newcommand{\DKLeIII}{\ensuremath{K_L\rightarrow\pi^\pm e^\mp\bar{\nu}(\nu)}}
\newcommand{\DKLmuIII}
           {\ensuremath{K_L\rightarrow\pi^\pm \mu^\mp\bar{\nu}(\nu)}}
\newcommand{\DKLmupmum}{\ensuremath{K_L\rightarrow\mu^+\mu^-}}
\newcommand{\DKLpipi}{\ensuremath{K_L\rightarrow\pi\pi}}
\newcommand{\DKLpippim}{\ensuremath{K_L\rightarrow\pi^+\pi^-}}
\newcommand{\DKLpippimpin}{\ensuremath{K_L\rightarrow\pi^+\pi^-\pi^0}}
\newcommand{\DKLpinpin}{\ensuremath{K_L\rightarrow\pi^0\pi^0}}
\newcommand{\DKLpinpinpin}{\ensuremath{K_L\rightarrow3\pi^0}}

\newcommand{\DKSgg}{\ensuremath{K_S\rightarrow\gamma\gamma}}
\newcommand{\DKSeIII}{\ensuremath{K_S\rightarrow\pi^\pm e^\mp\bar{\nu}(\nu)}}
\newcommand{\DKSpienu}{\ensuremath{K_S\rightarrow\pi e\nu}}
\newcommand{\DKSpinpin}{\ensuremath{K_S\rightarrow\pi^0\pi^0}}
\newcommand{\DKSpipi}{\ensuremath{K_S\rightarrow\pi\pi}}
\newcommand{\DKSpippim}{\ensuremath{K_S\rightarrow\pi^+\pi^-}}
\newcommand{\DKSpippimg}{\ensuremath{K_S\rightarrow\pi^+\pi^-\gamma}}
\newcommand{\DKSpippimrad}{\ensuremath{K_S\rightarrow\pi^+\pi^-(\gamma)}}
\newcommand{\DKSpippimpin}{\ensuremath{K_S\rightarrow\pi^+\pi^-\pi^0}}

\newcommand{\DKpmeIII}{\ensuremath{K^\pm_{e3}}}
\newcommand{\DKpmpipmpinpin}{\ensuremath{K^\pm\rightarrow\pi^\pm\pi^0\pi^0}}

\newcommand{\Domegaetag}{\ensuremath{\omega\rightarrow\eta\gamma}}
\newcommand{\Domegaping}{\ensuremath{\omega\rightarrow\pi^0\gamma}}

\newcommand{\Dphiazerog}{\ensuremath{\phi\rightarrow a_0\gamma}}
\newcommand{\Dphietaprg}{\ensuremath{\phi\rightarrow\eta'\gamma}}
\newcommand{\Dphietag}{\ensuremath{\phi\rightarrow\eta\gamma}}
\newcommand{\Dphietaping}{\ensuremath{\phi\rightarrow\eta\pi^0\gamma}}
\newcommand{\Dphifzerog}{\ensuremath{\phi\rightarrow f_0\gamma}}
\newcommand{\DphiKSKL}{\ensuremath{\phi\rightarrow K_S K_L}}
\newcommand{\Dphipinping}{\ensuremath{\phi\rightarrow\pi^0\pi^0\gamma}}
\newcommand{\Dphipippimpin}{\ensuremath{\phi\rightarrow\pi^+\pi^-\pi^0}}
\newcommand{\Dphirhonpin}{\ensuremath{\phi\rightarrow\rho^0\pi^0}}

\newcommand{\Dpimunu}{\ensuremath{\pi\rightarrow\mu\nu}}

\newcommand{\Drhonetag}{\ensuremath{\rho^0\rightarrow\eta\gamma}}
\newcommand{\Drhonping}{\ensuremath{\rho^0\rightarrow\pi^0\gamma}}

\newcommand{\EEgg}{\ensuremath{e^+e^-\rightarrow\gamma\gamma}}
\newcommand{\EEHadr}{\ensuremath{e^+e^-\rightarrow\mathrm{hadrons}}}
\newcommand{\EEepemg}{\ensuremath{e^+e^-\rightarrow e^+e^-\gamma}}
\newcommand{\EEmupmum}{\ensuremath{e^+e^-\rightarrow\mu^+\mu^-}}
\newcommand{\EEpippim}{\ensuremath{e^+e^-\rightarrow\pi^+\pi^-}}
\newcommand{\EEpippimg}{\ensuremath{e^+e^-\rightarrow\pi^+\pi^-\gamma}}
\newcommand{\EEomegapin}{\ensuremath{e^+e^-\rightarrow\omega\pi^0}}

